PAD: Personalized Alignment of LLMs at Decoding-Time

Aligning with personalized preferences, which vary significantly across cultural, educational, and political differences, poses a significant challenge due to the computational costs and data demands of traditional alignment methods. In response, this paper presents Personalized Alignment at Decoding-time (PAD), a novel framework designed to align LLM outputs with diverse personalized preferences during the inference phase, eliminating the need for additional training. By introducing a unique personalized reward modeling strategy, this framework decouples the text generation process from personalized preferences, facilitating the generation of generalizable token-level personalized rewards. The PAD algorithm leverages these rewards to guide the decoding process, dynamically tailoring the base model's predictions to personalized preferences. Extensive experimental results demonstrate that PAD not only outperforms existing training-based alignment methods in terms of aligning with diverse preferences but also shows significant generalizability to preferences unseen during training and scalability across different base models. This work advances the capability of LLMs to meet user needs in real-time applications, presenting a substantial step forward in personalized LLM alignment.

==> tab/method_evaluation.tex <==
\renewcommand{\arraystretch}{1.1}
\begin{table*}[t]
\caption{Comparison of baseline methods and PAD on predefined preferences. "–" indicates not applicable. The best result is highlighted in \textbf{bold}.}
\centering
  \resizebox{0.98\textwidth}{!}{
  \begin{tabular}{l|ccc|ccc|cc|cc}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c}{Helpful} & \multicolumn{3}{|c}{Harmless} & \multicolumn{2}{|c}{Humor} & \multicolumn{2}{|c}{Overall} \\
    \cmidrule(r){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
           & Armo & RM & GPT-4 & Armo & RM & GPT-4 & RM & GPT-4 & RM & GPT-4 \\
    \hline
    \multicolumn{11}{l}{\cellcolor[HTML]{E8E8E8}\textbf{Psoups dataset}}\\
Base & 0.63 & 1.06 & - & 0.97 & 0.83 & - & -0.93 & - & 0.32 & - \\
MORLHF & 0.31 & 0.91 & 14\% & 0.88 & 0.84 & 4\% & 0.28 & 82\% & 0.68 & 33\% \\
MODPO & 0.56 & 0.89 & 52\% & 0.96 & 0.77 & 80\% & -0.90 & 72\% & 0.25 & 68\% \\
Personalized soups & 0.38 & -0.72& 72\%& 0.92& 0.73& 92\%& -0.30& 80\%& -0.09& 81\% \\
Rewarded soups & 0.50 & 0.87 & 34\% & 0.95 & 0.87 & 64\% & 0.14 & 78\% & 0.63 & 59\% \\
RiC & 0.54 & 0.90 & 40\% & 0.97 & 0.90 & 70\% & -0.08 & 76\% & 0.58 & 62\% \\
Preference Prompting & 0.56 & 0.82 & 70\% & 0.96 & 0.87 & 90\% & -0.79 & 74\% & 0.30 & 78\% \\
MetaAligner & 0.55 & \textbf{1.39} & 66\% & 0.89 & 0.54 & 74\% & -0.97 & 74\% & 0.32 & 71\% \\
MOD & 0.55 & 0.93 & 60\% & 0.96 & 0.92 & 84\% & 0.38 & 78\% & 0.74 & 74\% \\
\revise{Aligner}              & \textbf{0.67} & 1.32  & 72\% & 0.97 & 0.63  & 70\% & -1.39 & 12\% & 0.19  & 51\% \\
\revise{Steering}             & 0.63 & 1.17  & 38\% & 0.96 & 0.81  & 66\%          & 0.17  & 70\% & 0.72  & 58\% \\
Args & - & 1.09 & \textbf{74\%} & - & 0.98 & \textbf{94\%} & - & - & - & - \\
\midrule
\model~(Ours) & 0.65 & 1.34 & \textbf{74\%} & \textbf{0.98} & \textbf{1.03} & 92\% & \textbf{0.82} & \textbf{86\%} & \textbf{1.06} & \textbf{84\%}
\\\hline
\multicolumn{11}{l}{\cellcolor[HTML]{E8E8E8}\textbf{HelpSteer dataset}}\\
Base & 0.57 & 0.56 & - & 0.98 & 0.5 & - & -0.56 & - & 0.17 & - \\
MORLHF & 0.49 & 0.6 & 52\% & 0.92 & 0.54 & 60\% & 0.15 & 62\% & 0.43 & 58\% \\
MODPO & 0.53 & 0.38 & 28\% & 0.99 & 0.69 & 76\% & -0.78 & 52\% & 0.10 & 52\% \\
Personalized soups & 0.42& -0.53& 54\%& 0.93& 0.66& 70\%& 0.14& 80\%& 0.09& 68\% \\
Rewarded soups & 0.52 & 0.63 & 46\% & 0.90 & 0.66 & 60\% & 0.00 & 48\% & 0.43 & 51\% \\
RiC & 0.51 & 0.66 & 38\% & \textbf{1.00} & 0.68 & 70\% & 0.01 & 68\% & 0.44 & 59\% \\
Preference Prompting & 0.52 & 0.52 & 56\% & 0.84 & 0.96 & 82\% & -0.49 & 86\% & 0.33 & 75\% \\
MetaAligner & 0.51 & \revise{\textbf{1.13}} & 58\% & 0.90 & 0.23 & 82\% & -0.69 & 76\% & 0.22 & 72\% \\
MOD & 0.50 & 0.66 & 56\% & 0.97 & 0.78 & 70\% & 0.24 & 52\% & 0.56 & 59\% \\
\revise{Aligner}              & 0.59 & 0.88 & 54\% & 0.99 & 0.44  & 90\%          & -0.77 & 8\%  & 0.18 & 51\% \\
\revise{Steering}            & 0.49 & 0.68 & 40\% & 0.88 & 0.7   & 72\% & 0.18  & 70\% & 0.52 & 61\% \\
Args & - & 0.86 & 50\% & - & 0.82 & 74\% & - & - & - & - \\
\midrule
\model~(Ours) & \textbf{0.65} & 0.89 & \textbf{62\%} & 0.94 & \textbf{0.99} & \textbf{86\%} & \textbf{1.01} & \textbf{92\%} & \textbf{0.96} & \textbf{80\%} \\\bottomrule
  \end{tabular}}
    \label{tab:methods_evaluation}
\end{table*}

==> tex/3_method.tex <==
\section{Method}

\subsection{Preliminaries}

In this section, we first define the per-token Markov Decision Process (MDP) for large language models (LLMs) and then describe its relationship to classic Reinforcement Learning from Human Feedback (RLHF) approaches.

\paragraph{Text generation as token-level markov decision process.}

We define the standard text generation process of large language models (LLMs) with prompt $\bx$ and response $\by$ as token-level Markov Decision Process (MDP). MDP is denoted as a tuple $\mathcal{M} = (\mathcal{S}, \mathcal{A}, \mathcal{P}, R)$, where the state space $\mathcal{S}$ consists of the prompt and all tokens generated so far (i.e., $\bs_t= (\bx, \by_{1:t-1})$). The action space $\mathcal{A}$ is the tokens from the vocabulary (i.e., $\ba_t = \by_t$). $\mathcal{P}$ is the transition kernel, which is deterministic that given state $\bs_t= (\bx, \by_{1:t-1})$ and action $\ba_t = \by_t$, the next state is $\bs_{t+1}= (\bs_{t}, \ba_t)= (\bx, \by_{1:t})$. R : $S \times A \to \mathbb{R}$ represents the reward at each step. Given an MDP, the goal is to maximise the expected return $G = \sum_{t=0}^{T} R_{t}, \text{ where } R_t = R(\bs_t, \ba_t)$. In order to do so the agent computes a (Markov) policy $\pi : S \to \Delta(A)$ that maps from state to a distribution over actions.

\iffalse
In RLHF, the reward function is learned from human feedback over preferences between responses which we will denote using trajectories $\tau$ at the token level. 
As is typically done \citep{ziegler2020finetuning, stiennon2022learning}, we assume that preference trajectories start at the same state (initial prompt) and end in a terminal state (\textbf{EOS} token), from which future rewards are zero. 
While the reward function $r$ will ultimately be learned from feedback, we assume that within the token-MDP the reward $r$ at terminal states must be zero. Note that this is not a restrictive assumption, as $r(\bs_t, \ba_t)$ can fully represent any reward dependent on the next state $\bs_{t+1}$ per the deterministic dynamics. 
In this token level MDP, the corresponding Bradley-Terry preference model is 
\begin{equation}\label{eq:dense-bradley-terry}
    p^*(\tau^w \succeq \tau^l)=\frac{\exp\left(\sum_{i=1}^N r(\bs_i^w, \ba_i^w)\right)}{\exp\left(\sum_{i=1}^N r(\bs_i^w, \ba_i^w)\right)+ \exp\left(\sum_{i=1}^M r(\bs_i^l, \ba_i^l)\right)}.
\end{equation}
which gives the probability that the ``win'' trajectory $\tau^w$ of length $N$ is preferred to the ``loss'' trajectory $\tau^l$ of length $M$. Now that we have defined the token level MDP, we can show how it relates to both classic and direct alignment RLHF methods.

In current RLHF theory, the agent’s objective is to maximize an observed reward function, with the optimal policy typically being deterministic and reward-greedy.
\fi

\paragraph{\wchai{rlhf first?} The RLHF Pipeline.}
 
Classic RLHF approaches first learn a reward function from human feedback on prompt and response pairs $(\bx, \by^w, \by^l)$. The reward function is modeled as a contextual bandit using Bradley-Terry preference model:

\begin{equation}
\label{eq:bandit_pref}
    p^*(\by^w \succeq \by^l) = \frac{\exp R(\bx,\by^w)} {\exp R(\bx,\by^w) + \exp R(\bx,\by^l)},
\end{equation}

where $\by^w$ and $\by^l$ denote the preferred and not-preferred completions for the prompt $\bx$. $p^*(\by^w \succeq \by^l)$ denotes the probability that $\by^w$ is preferred to $\by^l$.
Then, the policy model (i.e., the language model) $\pi_{\theta}$ is optimized with a gradient-based method like PPO with an entropy-bonus using the following KL-constrained RL objective:

\begin{equation}\label{eq:multi_step_RL}
\max_{\pi_{\theta}}  \mathbb{E}_{a_t \sim \pi_{\theta}(\cdot | \bs_t)}\left[\sum_{t=0}^T
(R(\bs_t, \ba_t) - \beta\mathcal{D}_{KL}(\pi_{\text{ref}}(\cdot
|\bs_t), \pi_{\theta}(\cdot
|\bs_t)) \right]
\end{equation}

\iffalse
\begin{equation}\label{eq:multi_step_RL}
\max_{\pi_{\theta}}  \mathbb{E}_{a_t \sim \pi_{\theta}(\cdot | \bs_t)}\left[\sum_{t=0}^T
(R(\bs_t, \ba_t) + \underbrace{\beta\log\pi_{\text{ref}}(\ba_t
|\bs_t)}_{\text{KL penalty}}) + \beta\mathcal{H}(\pi_{\theta})|\bs_0\sim\rho(\bs_0)\right]
\end{equation}
\fi

where $\pi_{\text{ref}}$ is a reference policy, often the language model resulting from supervised finetuning, from which the learned policy should not significantly deviate. In the optimization of the policy, only generating the EOS token carries a reward as output by the reward model which is combined with KL penalty, while for all other tokens in the vocabulary, only the KL component is non-zero. Additionally, it is worth mentioning that we omit the supervised finetuning (SFT) stage, which is often considered as part of the RLHF pipeline. This is due to that the SFT stage is not directly relevant to the focus of this paper.

% 此外，值得一提的是，我们在这里省略了supervised finetuning （SFT） stage, which经常被considered as part of RLHF Pipeline.这主要是由于SFT stage与本文关系不大。
\paragraph{Personalized alignment within MDP}
Unlike the unidirectional reward in traditional MDPs, we posit that personalized preferences may vary across different dimensions; for example, some users may prefer concise and understandable responses, while others might favor comprehensive and expert answers. In this way, we define the reward function of personalized alignment as $\hat{R} : S \times A \to \mathbb{R}^n$, which describes a vector of n rewards, one for each dimension of personalized preference (e.g, concise/comprehensive, expert/elementary), instead of a scalar. During alignment, a personalized preference may encompass one or several dimensions of rewards.

Based on this, existing work~\citep{li2020deep, rame2024rewarded} employs a linear scalarization strategy, denoting human preferences as $w$ such that $ R= w^T \hat{R}$. Subsequently, this approach optimizes the policy with RLHF objective or performs a weighted merging of multiple policies. However, such approaches still cannot overcome the high time and computational costs associated with optimizing the policy (i.e., the language model).

\begin{figure}[t]
	\centering
	\includegraphics[width=1.\linewidth]{fig/Personalized_Decoding_Pipeline.pdf}
	\caption{An illustration of our framework. \wchai{Which part of the parameters can be updated?}}
    \label{fig:pipeline}
\end{figure}


\subsection{Personalized alignment as value-guided search}

In this section, we propose Personalized Alignment at Decoding-Time (\model), a novel approach that does not require training a policy and is transferable to diverse personalized preferences. Inspired by the concept of successor features~\citep{dayan1993improving,barreto2017successor}, we first define personalized rewards, which decouple the features of the current state from personalized preferences. Next, we define the value function, which is composed of the dynamics induced by the language model and the personalized preferences. Finally, we introduce our value-guided decoding algorithm, which aligns with personalized preferences by utilizing the value function for weighting during the inference phase.


\begin{definition}
\label{personalized reward function}
A \textbf{personalized reward function} R that,
\begin{equation}
    R(\bs, \ba) = \bw_p^{\top}\phi(\bs,\ba),
\end{equation}
where $\phi(\bs,\ba) \in \mathbb{R}^d$ are features of $(\bs,\ba)$ and $\bw_p \in \mathbb{R}^d$ are weights toward a certain personalized preference 
$p$. In order to build some intuition, it helps to think of $\phi(\bs,\ba)$ as salient events that may be desirable or undesirable to the agent. 

\end{definition}

Thus, personalized reward is deterministic given a deterministic personalized preference. Therefore, the goal of personalized alignment is to find a optimal policy that maximizes the personalized reward.
In this way, the personalized preferences are captured by the weights \(\bw_p\). The weights \(\bw_p\) are independent of the current state and action, thus they can be decoupled from the MDP dynamics. When the user's personalized preferences change, only \(\bw_p\) needs to be modified to obtain the personalized reward.


Based on Definition~\ref{personalized reward function}, personalized reward model can be optimized by modifying Equation~\ref{eq:bandit_pref}:
\begin{equation}
\label{loss_reward}
\mathcal{L}_\phi(D) = -\mathbb{E}_{(x, y_w, y_l) \sim D} \left[ \log \sigma \left( \bw_p^{\top} (\phi(x, y_w) - \phi(x, y_l)) \right) \right].
\end{equation}

With the reward model $R = w_p^{\top}\phi(x, y)$, traditional RLHF paradigm requires optimizing a policy (training the language model) for each personalized preference or jointly optimizing a policy for multiple personalized preferences, which is resource-intensive or challenging.
%已有RLHF方法是如何寻找optimal policy的

To tackle this problem, we consider an value-iterating alternative~\citep{watkins1992q} of policy optimization (e.g., PPO) to solve the optimal policy.
We first consider the action-value function (i.e., Q function) $Q$ based on the token-level reward $R^{\pi}(\bw_p, \bs, \ba)$:

\begin{equation}
\label{personalized Q}
    Q^{\pi}(\bw_p, \bs_t, \ba_t) = \bw_p^{\top} \mathbb{E} [\sum_{i=t}^{T} \phi(\bs_i,\ba_i)| \ba_i \sim \pi_{LM} (\cdot|\bs_i)] = \bw_p^{\top} \psi^{\pi}(\bs_t, \ba_t),
\end{equation}
where $\mathbb{E}$ is the expectation is over the randomness due to the sampling from the base language model $\pi_{LM}$. $Q$ function models the total future reward from $(\bs, \ba)$ under $\pi$. With $Q$ function, we can obtain the same optimal policy $\pi^*$ as in Equation~\ref{eq:multi_step_RL} by:

\begin{equation}
    \pi^*(\ba_t|\bs_t, \bw_p) = e^{(Q^*(\bw_p, \bs_t,\ba_t)-V^*(\bw_p, \bs_t))/\beta},
\end{equation}
where $V$ is the corresponding state-value function at current state. Thus we formulate the optimal policy as selecting the action that maximizes the soft $Q^*$ function. This formulates the alignment of large language models (LLMs) as a $Q^*$ guided search at decoding time.

To obtain the $Q^*$ function, we begin by rewrite the reward as in \citet{rafailov2024direct}.
Assume that there exists $\hat{\pi}(y|x)$, which represents a vector of probabilities of y in terms of $|\bw_p|$ dimensions, that satisfies:
\begin{equation}
r (x, y) = \bw_p^{\top}\phi(x, y) = \bw_p^{\top} \beta \log \frac{\hat{\pi}_{\theta}(y|x)}{\hat{\pi}_{\text{ref}}(y|x)} = \frac{{\pi}_{\theta}(y|x)}{{\pi}_{\text{ref}}(y|x)} \\
\end{equation}

Substituting this relationship into Eq.~\ref{loss_reward}:
\begin{equation}
\label{finalloss}
\mathcal{L}_\theta(D) = -\mathbb{E}_{(x, y_w, y_l) \sim D} \left[ \log \sigma \left( \bw_p^{\top} (\beta\log\frac{\hat{\pi}_{\theta}(y_w|x)}{\hat{\pi}_{\text{ref}}(y_w|x)} - \beta\log\frac{\hat{\pi}_{\theta}(y_l|x)}{\hat{\pi}_{\text{ref}}(y_l|x)}) \right) \right].
\end{equation}

We then replace the sentence-level reward function in (2.1) with token-wise reward functions as done in \citet{rafailov2024direct}:

\begin{equation}
\phi(x, y) := \beta \log \frac{\hat{\pi}_{\theta}(y|x)}{\hat{\pi}_{\text{ref}}(y|x)} = \beta \sum_{t=1}^{T} \log \frac{\hat{\pi}_{\theta}(\ba_t | \bs_t)}{\hat{\pi}_{\text{ref}}(\ba_t | \bs_t)} = \sum_{t=1}^{T} \phi(\bs, \ba).\\
\end{equation}

At $t=T$, we have $\psi^{*}(\bs_T, \ba_T) = \phi(x, y) = \beta \sum_{t=1}^{T} \log \frac{\hat{\pi}_{\theta}(\ba_t | \bs_t)}{\hat{\pi}_{\text{ref}}(\ba_t | \bs_t)}$. Substituting into Eq.~\ref{personalized Q}, we have

\begin{equation}
\label{Qfunction}
Q^{*}(\bw_p, \bs_t, \ba_t) =  \bw_p^{\top}\psi^{*}(\bs_t, \ba_t) = \bw_p^{\top} \beta \sum_{i=1}^{t} \log \frac{\hat{\pi}_{\theta}(\ba_i | \bs_i)}{\hat{\pi}_{\text{ref}}(\ba_i | \bs_i)}. \\
\end{equation}

\begin{definition}
\textbf{Personalized alignment at decoding-time (\model)} can be formally defined as solving for the optimal decoding policy $\pi^*(\bs)$ under the token level MDP M. The optimal policy can be determined by selecting the action that maximizes $A^{*}$ at each step:
\begin{align}
\label{\modelfuntion}
    \pi_{\model}^*(\ba | \bs_t, \bw_p) & \propto \pi_{LM}^*(\ba | \bs_t, \bw_p) e^{\beta(Q^{*}(\bw_p,\bs_t,\ba)-V^{*}(\bw_p,\bs_t))}.
\end{align}
\end{definition}

Note that different from RLHF framework that directly models the LLM as policy, our policy selects action that maximizes $\Delta Q^{*}$ at each step.

\subsection{Generalized personalized alignment}

In this section, we discuss the ability of~\model~to transfer to unseen personalized preferences. Suppose now that we have computed optimal value function for n personalized preferences \(w_1, w_2, \ldots, w_n \in w^\phi\), denoted as \(\{Q^{*}_{1}, Q^{*}_{2}, \ldots, Q^{*}_{n}\}\).
Now, if the reward changes to $r_{n+1}(s,a) = w_{n+1}^\top \phi(s,a) $, as long as we have $w_{n+1}$ we can compute the new value function of $\pi_i^*$ by simply making $Q_{n+1}^{*}(s,a) = w_{n+1}^\top \psi^{*}(s,a) $. Once the functions $Q_{n+1}^{*}$ have been computed, we can we can apply generalized policy improvement~\citep{bellman1966dynamic, barreto2017successor} to estimate its performance on $w_{n+1}$.


\textbf{Theorem 1.} Let $\bw_i \in \mathcal{W}^\phi$ and let $Q_i^{*}$ be the action-value function of an optimal policy of $\bw_i$. 
for all $\bs \in \mathcal{S}$, $\ba \in \mathcal{A}$, and $j \in \{ 1, 2, \dots, n \}$, let $\pi(\bs) \in \arg\max_a \max_i Q_i^{*}(\bs, \ba)$. Finally, let $\phi_{\max} = \max_{\bs,\ba} \| \phi(\bs,\ba) \|$, where $\| \cdot \|$ is the norm induced by the inner product adopted. Then,
\[
Q_{n+1}^{\pi^*}(\bs, \ba) - Q_{n+1}^{\pi}(\bs, \ba) \leq |H| \left( \phi_{\max} \min_j \| \mathbf{w}_{n+1} - \mathbf{w}_j \|\right).
\]

This term is a multiple of the distance between \(\bw_i\) and the closest \(\bw_j\) for which we have already computed a policy. The formula formalizes the intuition that if the agent has previously solved a similar task, it should perform well on task \(\bw_i\).


\subsection{Practical Implementations}

In this section, we introduce the practical implementation of the training and inference of Personalized Alignment at Decoding-time (\model). 

\paragraph{Optimization}
We consider utilizing an LLM-based model to predict the features $\phi$ and preferences $w_p$. For simplicity, we employ a single backbone to model $\phi$ and then utilize an additional prediction head to derive $w_p$. The optimization occurs in two phases with Equation~\ref{finalloss}. In the first phase, we fix $w_p$ as a unit vector and optimize the backbone to learn general features. In the second phase, we freeze the backbone and only optimize the prediction head for $w_p$ to learn different user preferences.


\paragraph{Value-guided decoding}
In the inference phase, given the personalized preference $p$ the previous context $s = (x, y_{<t})$ at step $t$, the advantage function $r(\bw_p,\bs_t,\ba) = \beta(Q^{*}(\bw_p,\bs_t,\ba)-V^{*}(\bw_p,\bs_t)$ for the token $\ba$ can be calculated using Equation~\ref{Qfunction}. Subsequently, according to Equation~\ref{\modelfuntion}, the output logits distribution can be obtained by combining the probability distribution of the base model and the advantage value:

\begin{align}
\pi^*_{\text{\model}}(\cdot | s_t) := \arg\max_{a_t} \mathbb{E}_{a_t \sim \pi_{LM}(\cdot | s_t)} \left[  \beta w_p^{\top}  \log \frac{\hat{\pi}_{\theta}(\ba_t | \bs_t)}{\hat{\pi}_{\text{ref}}(\ba_t | \bs_t)}  + \pi_{LM}(\cdot | s_t)\right].
\end{align}


==> tex/3_methodv2.tex <==
\section{Method}

\subsection{Preliminaries}

In this section, we first define the per-token Markov Decision Process (MDP) for large language models (LLMs) and then describe its relationship to classic Reinforcement Learning from Human Feedback (RLHF) approaches.

\paragraph{Text generation as token-level markov decision process.}

We define the standard text generation process of large language models (LLMs) with prompt $\bx$ and response $\by$ as token-level Markov Decision Process (MDP). MDP is denoted as a tuple $\mathcal{M} = (\mathcal{S}, \mathcal{A}, \mathcal{P}, R)$, where the state space $\mathcal{S}$ consists of the prompt and all tokens generated so far (i.e., $\bs_t= (\bx, \by_{1:t-1})$). The action space $\mathcal{A}$ is the tokens from the vocabulary (i.e., $\ba_t = \by_t$). $\mathcal{P}$ is the transition kernel, which is deterministic that given state $\bs_t= (\bx, \by_{1:t-1})$ and action $\ba_t = \by_t$, the next state is $\bs_{t+1}= (\bs_{t}, \ba_t)= (\bx, \by_{1:t})$. R : $S \times A \to \mathbb{R}$ represents the reward at each step. Given an MDP, the goal is to maximise the expected return $G = \sum_{t=0}^{T} R_{t}, \text{ where } R_t = R(\bs_t, \ba_t)$. In order to do so the agent computes a (Markov) policy $\pi : S \to \Delta(A)$ that maps from state to a distribution over actions.

\iffalse
In RLHF, the reward function is learned from human feedback over preferences between responses which we will denote using trajectories $\tau$ at the token level. 
As is typically done \citep{ziegler2020finetuning, stiennon2022learning}, we assume that preference trajectories start at the same state (initial prompt) and end in a terminal state (\textbf{EOS} token), from which future rewards are zero. 
While the reward function $r$ will ultimately be learned from feedback, we assume that within the token-MDP the reward $r$ at terminal states must be zero. Note that this is not a restrictive assumption, as $r(\bs_t, \ba_t)$ can fully represent any reward dependent on the next state $\bs_{t+1}$ per the deterministic dynamics. 
In this token level MDP, the corresponding Bradley-Terry preference model is 
\begin{equation}\label{eq:dense-bradley-terry}
    p^*(\tau^w \succeq \tau^l)=\frac{\exp\left(\sum_{i=1}^N r(\bs_i^w, \ba_i^w)\right)}{\exp\left(\sum_{i=1}^N r(\bs_i^w, \ba_i^w)\right)+ \exp\left(\sum_{i=1}^M r(\bs_i^l, \ba_i^l)\right)}.
\end{equation}
which gives the probability that the ``win'' trajectory $\tau^w$ of length $N$ is preferred to the ``loss'' trajectory $\tau^l$ of length $M$. Now that we have defined the token level MDP, we can show how it relates to both classic and direct alignment RLHF methods.

In current RLHF theory, the agent’s objective is to maximize an observed reward function, with the optimal policy typically being deterministic and reward-greedy.
\fi

\paragraph{\wchai{rlhf first?} The RLHF Pipeline.}
 
Classic RLHF approaches first learn a reward function from human feedback on prompt and response pairs $(\bx, \by^w, \by^l)$. The reward function is modeled as a contextual bandit using Bradley-Terry preference model:

\begin{equation}
\label{eq:bandit_pref}
    p^*(\by^w \succeq \by^l) = \frac{\exp R(\bx,\by^w)} {\exp R(\bx,\by^w) + \exp R(\bx,\by^l)},
\end{equation}

where $\by^w$ and $\by^l$ denote the preferred and not-preferred completions for the prompt $\bx$. $p^*(\by^w \succeq \by^l)$ denotes the probability that $\by^w$ is preferred to $\by^l$.
Then, the policy model (i.e., the language model) $\pi_{\theta}$ is optimized with a gradient-based method like PPO with an entropy-bonus using the following KL-constrained RL objective:

\begin{equation}\label{eq:multi_step_RL}
\max_{\pi_{\theta}}  \mathbb{E}_{a_t \sim \pi_{\theta}(\cdot | \bs_t)}\left[\sum_{t=0}^T
(R(\bs_t, \ba_t) - \beta\mathcal{D}_{KL}(\pi_{\text{ref}}(\cdot
|\bs_t), \pi_{\theta}(\cdot
|\bs_t)) \right]
\end{equation}

\iffalse
\begin{equation}\label{eq:multi_step_RL}
\max_{\pi_{\theta}}  \mathbb{E}_{a_t \sim \pi_{\theta}(\cdot | \bs_t)}\left[\sum_{t=0}^T
(R(\bs_t, \ba_t) + \underbrace{\beta\log\pi_{\text{ref}}(\ba_t
|\bs_t)}_{\text{KL penalty}}) + \beta\mathcal{H}(\pi_{\theta})|\bs_0\sim\rho(\bs_0)\right]
\end{equation}
\fi

where $\pi_{\text{ref}}$ is a reference policy, often the language model resulting from supervised finetuning, from which the learned policy should not significantly deviate. In the optimization of the policy, only generating the EOS token carries a reward as output by the reward model which is combined with KL penalty, while for all other tokens in the vocabulary, only the KL component is non-zero. Additionally, it is worth mentioning that we omit the supervised finetuning (SFT) stage, which is often considered as part of the RLHF pipeline. This is due to that the SFT stage is not directly relevant to the focus of this paper.

% 此外，值得一提的是，我们在这里省略了supervised finetuning （SFT） stage, which经常被considered as part of RLHF Pipeline.这主要是由于SFT stage与本文关系不大。
\paragraph{Personalized alignment within MDP}
Unlike the unidirectional reward in traditional MDPs, we posit that personalized preferences may vary across different dimensions; for example, some users may prefer concise and understandable responses, while others might favor comprehensive and expert answers. In this way, we define the reward function of personalized alignment as $\hat{R} : S \times A \to \mathbb{R}^n$, which describes a vector of n rewards, one for each dimension of personalized preference (e.g, concise/comprehensive, expert/elementary), instead of a scalar. During alignment, a personalized preference may encompass one or several dimensions of rewards.

Based on this, existing work~\citep{li2020deep, rame2024rewarded} employs a linear scalarization strategy, denoting human preferences as $w$ such that $ R= w^T \hat{R}$. Subsequently, this approach optimizes the policy with RLHF objective or performs a weighted merging of multiple policies. However, such approaches still cannot overcome the high time and computational costs associated with optimizing the policy (i.e., the language model).

\begin{figure}[t]
	\centering
	\includegraphics[width=1.\linewidth]{fig/Personalized_Decoding_Pipeline.pdf}
	\caption{An illustration of our framework. \wchai{Which part of the parameters can be updated?}}
    \label{fig:pipeline}
\end{figure}


\subsection{Personalized alignment as value-guided search}

In this section, we propose Personalized Alignment at Decoding-Time (\model), a novel approach that does not require training a policy and is transferable to diverse personalized preferences. Inspired by the concept of successor features~\citep{dayan1993improving,barreto2017successor}, we first define personalized rewards, which decouple the features of the current state from personalized preferences. Next, we define the value function, which is composed of the dynamics induced by the language model and the personalized preferences. Finally, we introduce our value-guided decoding algorithm, which aligns with personalized preferences by utilizing the value function for weighting during the inference phase.


\begin{definition}
\label{personalized reward function}
A \textbf{personalized reward function} R can be represented by:
\begin{equation}
\label{personalized reward function}
    R(p, \bs, \ba) = \bw_p^{\top}\phi(\bs,\ba),
\end{equation}
where $\phi(\bs,\ba) \in \mathbb{R}^d$ are features of $(\bs,\ba)$ and $\bw_p \in \mathbb{R}^d$ are weights toward a certain personalized preference 
$p$. 
\end{definition}
The vector \(\bw_p\) models \(p\) as the degree of importance for each dimension of \(\phi(\bs,\ba)\). In this manner, \(\bw_p\) is independent of \((\bs,\ba)\), thereby allowing it to be decoupled from the MDP dynamics. When the user's personalized preferences change, only \(\bw_p\) are altered, which in turn modifies the \(R(p, \bs, \ba)\).
Consequently, the goal of personalized alignment can be defined as obtaining the policy that maximizes the personalized reward for each \(p\).

To address the resource-intensive nature of existing policy optimization methods, we consider a value-iteration alternative~\citep{watkins1992q} to derive the optimal policy.
We are inspired by that the optimal policy $\pi^*$ obtained by Equation~\ref{eq:multi_step_RL} can be formulated as~\cite{ziebart2010modeling, rafailov2024r}:

\begin{equation}
    \pi^*(\ba_t|\bs_t, p) = e^{(Q^*(p, \bs_t,\ba_t)-V^*(p, \bs_t))/\beta},
\end{equation}
where $Q$, the action-value function (i.e., Q function) based on the token-level reward $R^{\pi}(p, \bs, \ba)$, models the total future reward from $(\bs, \ba)$ under policy $\pi$. $V$ is the corresponding state-value function at current state:
\begin{align}
    Q^{\pi}(p, \bs_t, \ba_t) &= \mathbb{E} [\sum_{i=t}^{T} R(p, \bs_i,\ba_i)| \ba_i \sim \pi (\cdot|\bs_i)], \label{eq:Q_function} \\
    V^{\pi}(p, \bs_t) &= \beta \log \left( \int_{\mathcal{A}} e^{Q^{\pi}(p, \bs_t, \ba_t)/\beta} \, d\ba \right),
\end{align}
where $\mathbb{E}$ is the expectation is over the randomness due to the sampling from the base language model $\pi$. $Q^*$ denotes the Q funtion under optimal policy $\pi^{*}$.
Substitute Eq.~\ref{personalized reward function} into Eq.~\ref{eq:Q_function}, we can express $Q$ function as:
\begin{align}
\label{personalized Q}
    Q^{\pi}(p, \bs_t, \ba_t) &= \bw_p^{\top} \mathbb{E} [\sum_{i=t}^{T} \phi(\bs_i,\ba_i)| \ba_i \sim \pi (\cdot|\bs_i)] = \bw_p^{\top} \psi^{\pi}(\bs_t, \ba_t).
\end{align}

To obtain the $Q^*$ function, we begin by rewrite the reward as in \citet{rafailov2024direct}.
Assume that there exists $\hat{\pi}(y|x)$, which represents a vector of probabilities of y in terms of $|\bw_p|$ dimensions, that satisfies:
\begin{equation}
R (p, x, y) = \bw_p^{\top}\phi(x, y) = \bw_p^{\top} \beta \log \frac{\hat{\pi}_{\theta}(y|x)}{\hat{\pi}_{\text{ref}}(y|x)} = \frac{{\pi}_{\theta}(y|x)}{{\pi}_{\text{ref}}(y|x)} \\
\end{equation}

Substituting this relationship into Eq.~\ref{loss_reward}:
\begin{equation}
\label{finalloss}
\mathcal{L}_\theta(D) = -\mathbb{E}_{(x, y_w, y_l) \sim D} \left[ \log \sigma \left( \bw_p^{\top} (\beta\log\frac{\hat{\pi}_{\theta}(y_w|x)}{\hat{\pi}_{\text{ref}}(y_w|x)} - \beta\log\frac{\hat{\pi}_{\theta}(y_l|x)}{\hat{\pi}_{\text{ref}}(y_l|x)}) \right) \right].
\end{equation}

We then replace the sentence-level reward function in (2.1) with token-wise reward functions as done in \citet{rafailov2024direct}:

\begin{equation}
\phi(x, y) := \beta \log \frac{\hat{\pi}_{\theta}(y|x)}{\hat{\pi}_{\text{ref}}(y|x)} = \beta \sum_{t=1}^{T} \log \frac{\hat{\pi}_{\theta}(\ba_t | \bs_t)}{\hat{\pi}_{\text{ref}}(\ba_t | \bs_t)} = \sum_{t=1}^{T} \phi(\bs, \ba).\\
\end{equation}

At $t=T$, we have $\psi^{*}(\bs_T, \ba_T) = \phi(x, y) = \beta \sum_{t=1}^{T} \log \frac{\hat{\pi}_{\theta}(\ba_t | \bs_t)}{\hat{\pi}_{\text{ref}}(\ba_t | \bs_t)}$. Substituting into Eq.~\ref{personalized Q}, we have

\begin{equation}
\label{Qfunction}
Q^{*}(p, \bs_t, \ba_t) =  \bw_p^{\top}\psi^{*}(\bs_t, \ba_t) = \bw_p^{\top} \beta \sum_{i=1}^{t} \log \frac{\hat{\pi}_{\theta}(\ba_i | \bs_i)}{\hat{\pi}_{\text{ref}}(\ba_i | \bs_i)}. \\
\end{equation}

Finally, we formulate the personalized alignment as a $Q^*$ guided search at decoding time.

\begin{definition}
\textbf{Personalized alignment at decoding-time (\model)} can be formally defined as solving for the optimal decoding policy $\pi^*(\bs)$ under the token level MDP M. The optimal policy can be determined by selecting the action that maximizes $A^{*}$ at each step:
\begin{align}
\label{\modelfuntion}
    \pi_{\model}^*(\ba | \bs_t, p) & \propto \pi_{LM}(\ba | \bs_t, p) e^{\beta(Q^{*}(p,\bs_t,\ba)-V^{*}(p,\bs_t))}.
\end{align}
\end{definition}

Note that different from RLHF framework that directly models the LLM as policy, our policy selects action that maximizes $\Delta Q^{*}$ at each step.

\subsection{Generalized personalized alignment}

In this section, we discuss the ability of~\model~to transfer to unseen personalized preferences. Suppose now that we have computed optimal value function for n personalized preferences \(\bw_1, \bw_2, \ldots, \bw_n \in \bw^\phi\), denoted as \(\{Q^{*}_{1}, Q^{*}_{2}, \ldots, Q^{*}_{n}\}\).
Now, if the reward changes to $R(p_{n+1},\bs,\ba) = \bw_{n+1}^\top \phi(\bs,\ba) $, as long as we have $\bw_{n+1}$ we can compute the new value function of $\pi_i^*$ by simply making $Q_{n+1}^{*}(\bs,\ba) = \bw_{n+1}^\top \psi^{*}(\bs,\ba) $. Once the functions $Q_{n+1}^{*}$ have been computed, we can we can apply generalized policy improvement~\citep{bellman1966dynamic, barreto2017successor} to estimate its performance on $\bw_{n+1}$.


\textbf{Theorem 1.} Let $\bw_i \in \mathcal{W}^\phi$ and let $Q_i^{*}$ be the action-value function of an optimal policy of $\bw_i$. 
for all $\bs \in \mathcal{S}$, $\ba \in \mathcal{A}$, and $j \in \{ 1, 2, \dots, n \}$, let $\pi(\bs) \in \arg\max_a \max_i Q_i^{*}(\bs, \ba)$. Finally, let $\phi_{\max} = \max_{\bs,\ba} \| \phi(\bs,\ba) \|$, where $\| \cdot \|$ is the norm induced by the inner product adopted. Then,
\[
Q_{n+1}^{\pi^*}(p_{n+1}, \bs, \ba) - Q_{n+1}^{\pi}(p, \bs, \ba) \leq |H| \left( \phi_{\max} \min_j \| \mathbf{w}_{p_{n+1}} - \mathbf{w}_{p_j} \|\right).
\]

This term is a multiple of the distance between \(\bw_i\) and the closest \(\bw_j\) for which we have already computed a policy. The formula formalizes the intuition that if the agent has previously solved a similar task, it should perform well on task \(\bw_i\).


\subsection{Practical Implementations}

In this section, we introduce the practical implementation of the training and inference of Personalized Alignment at Decoding-time (\model). 

\paragraph{Optimization}
We consider utilizing an LLM-based model to predict the features $\phi$ and preferences $\bw_p$. For simplicity, we employ a single backbone to model $\phi$ and then utilize an additional prediction head to derive $\bw_p$. The optimization occurs in two phases with Equation~\ref{finalloss}. In the first phase, we fix $\bw_p$ as a unit vector and optimize the backbone to learn general features. In the second phase, we freeze the backbone and only optimize the prediction head for $\bw_p$ to learn different user preferences.


\paragraph{Value-guided decoding}
In the inference phase, given the personalized preference $p$ the previous context $s = (x, y_{<t})$ at step $t$, the advantage function $R(p,\bs_t,\ba) = \beta(Q^{*}(p,\bs_t,\ba)-V^{*}(p,\bs_t)$ for the token $\ba$ can be calculated using Equation~\ref{Qfunction}. Subsequently, according to Equation~\ref{\modelfuntion}, the output logits distribution can be obtained by combining the probability distribution of the base model and the advantage value:

\begin{align}
\pi^*_{\text{\model}}(\cdot | \bs_t, p) := \arg\max_{a_t} \mathbb{E}_{a_t \sim \pi_{LM}(\cdot | \bs_t)} \left[  \beta \bw_p^{\top}  \log \frac{\hat{\pi}_{\theta}(\ba_t | \bs_t)}{\hat{\pi}_{\text{ref}}(\ba_t | \bs_t)}  + \pi_{LM}(\cdot | \bs_t)\right].
\end{align}


==> tex/3_methodv3.tex <==
\section{Method}

\subsection{Preliminaries}

In this section, we first define the per-token Markov Decision Process (MDP) for large language models (LLMs) and describe its relationship to classic Reinforcement Learning from Human Feedback (RLHF) approaches. Then, we describe the characteristics and challenges of personalized alignment.

\paragraph{Text generation as token-level markov decision process.}

The standard text generation process of large language models (LLMs) with prompt $\bx$ and response $\by$ can be defined as token-level Markov Decision Process (MDP). MDP is denoted as a tuple $\mathcal{M} = (\mathcal{S}, \mathcal{A}, \mathcal{P}, R, T)$, where the state space $\mathcal{S}$ consists of the prompt and all tokens generated so far (i.e., $\bs_t= (\bx, \by_{1:t-1})$). The action space $\mathcal{A}$ is the tokens from the vocabulary (i.e., $\ba_t = \by_t$). $\mathcal{P}$ is the transition kernel, which is deterministic that given state $\bs_t= (\bx, \by_{1:t-1})$ and action $\ba_t = \by_t$, the next state is $\bs_{t+1}= (\bs_{t}, \ba_t)= (\bx, \by_{1:t})$. R : $S \times A \to \mathbb{R}$ represents the reward at each step. The maximum token count, $T$, sets the length limit for LLM outputs, which conclude with an end-of-sentence (EoS) token $\by_T=$ EoS that ends the generation. Given an MDP, the objective is to maximize the expected return $R(\bx,\by) = \sum_{t=1}^{T}R(\bs_t, \ba_t)$. To achieve this, the agent computes a (Markov) policy $\pi : S \to \Delta(A)$ that maps from state to a distribution over actions.

\iffalse
In RLHF, the reward function is learned from human feedback over preferences between responses which we will denote using trajectories $\tau$ at the token level. 
As is typically done \citep{ziegler2020finetuning, stiennon2022learning}, we assume that preference trajectories start at the same state (initial prompt) and end in a terminal state (\textbf{EoS} token), from which future rewards are zero. 
While the reward function $r$ will ultimately be learned from feedback, we assume that within the token-MDP the reward $r$ at terminal states must be zero. Note that this is not a restrictive assumption, as $r(\bs_t, \ba_t)$ can fully represent any reward dependent on the next state $\bs_{t+1}$ per the deterministic dynamics. 
In this token level MDP, the corresponding Bradley-Terry preference model is 
\begin{equation}\label{eq:dense-bradley-terry}
    p^*(\tau^w \succeq \tau^l)=\frac{\exp\left(\sum_{i=1}^N r(\bs_i^w, \ba_i^w)\right)}{\exp\left(\sum_{i=1}^N r(\bs_i^w, \ba_i^w)\right)+ \exp\left(\sum_{i=1}^M r(\bs_i^l, \ba_i^l)\right)}.
\end{equation}
which gives the probability that the ``win'' trajectory $\tau^w$ of length $N$ is preferred to the ``loss'' trajectory $\tau^l$ of length $M$. Now that we have defined the token level MDP, we can show how it relates to both classic and direct alignment RLHF methods.

In current RLHF theory, the agent’s objective is to maximize an observed reward function, with the optimal policy typically being deterministic and reward-greedy.
\fi

\paragraph{The RLHF Pipeline.}
 
Classic RLHF approaches~\cite{ziegler2019fine} first learn a reward function from human feedback on prompt and response pairs $(\bx, \by^w, \by^l)$. The reward function is modeled under a contextual bandit setting using the Bradley-Terry preference model~\cite{bradley1952rank}:
\begin{equation}
\label{eq:bandit_pref}
    p^*(\by^w \succeq \by^l) = \frac{\exp R(\bx,\by^w)} {\exp R(\bx,\by^w) + \exp R(\bx,\by^l)},
\end{equation}

where $\by^w$ and $\by^l$ denote the preferred and not-preferred completions for the prompt $\bx$. $p^*(\by^w \succeq \by^l)$ denotes the probability that $\by^w$ is preferred to $\by^l$.
The reward model can be learned through Maximal Likelihood Estimation (MLE) on this dataset D:
\begin{equation}
\label{eq:reward modeling}
    \mathcal{L}(R, D) = \mathbb{E}_{(\bx,\by_w,\by_l) \sim D} \left[ \log \sigma(R(\bx, \by_w) - R(\bx, \by_l)) \right].
\end{equation}

Then, we use the learned reward model to provide feedback. The policy model (i.e., the language model) $\pi_{\theta}$ is optimized with a gradient-based method like PPO~\cite{schulman2017proximal} with an entropy-bonus using the following KL-constrained RL objective:
\begin{equation}\label{eq:multi_step_RL}
\max_{\pi_{\theta}}  \mathbb{E}_{\by \sim \pi_{\theta}(\by| \bx)}\left[\sum_{t=0}^T
(R(\bx, \by) - \beta\mathcal{D}_{KL}(\pi_{\text{ref}}(
\by|\bx), \pi_{\theta}(\by
|\bx)) \right]
\end{equation}

where $\pi_{\text{ref}}$ represents a reference policy, typically the language model resulting from supervised fine-tuning, from which the learned policy should not significantly deviate. $\beta$ is a parameter used to control this deviation. In practice, the language model policy $\pi_{\theta}$ is initially set to $\pi_{\text{ref}}$. Additionally, it is important to note that we exclude the supervised fine-tuning (SFT) stage in the RLHF pipeline. This is due to that the SFT stage is not directly relevant to the focus of this paper.
% $\pi_{\text{ref}}$ is a reference policy, often the language model resulting from supervised finetuning, from which the learned policy should not significantly deviate. $\beta$ is a parameter controlling the deviation. In practice, the language model policy $\pi_{\theta}$ is also initialized to $\pi_{\text{ref}}$. Additionally, it is worth mentioning that we omit the supervised finetuning (SFT) stage, which is often considered as part of the RLHF pipeline. This is due to that the SFT stage is not directly relevant to the focus of this paper.

\paragraph{Personalized alignment within MDP}
Unlike the unidirectional reward in traditional MDPs, we posit that personalized preferences may vary across different dimensions; for example, some users may prefer concise and understandable responses, while others might favor comprehensive and expert answers. In this way, the reward function of personalized alignment can be defined as $\hat{R} : S \times A \to \mathbb{R}^n$, which describes a vector of n rewards, one for each dimension of personalized preference (e.g, concise/comprehensive, expert/elementary), instead of a scalar. During alignment, a personalized preference may encompass one or several dimensions of rewards.

Based on this, existing work~\citep{li2020deep, rame2024rewarded} employs a linear scalarization strategy, denoting human preferences as $w$ such that $ R= w^T \hat{R}$. Subsequently, these approaches optimize the policy with RLHF objective or perform a weighted merging of multiple policies.
\textit{However, these approaches still cannot overcome the high time and computational costs associated with optimizing the policy (i.e., the language model) for multiple personalized preferences simultaneously.}


\subsection{Personalized alignment at Decoding-time}

In this section, we propose Personalized Alignment at Decoding-Time (\model), a novel approach that does not require training a policy and is transferable to diverse personalized preferences. Inspired by the concept of successor features~\citep{dayan1993improving,barreto2017successor}, we first define the personalized reward function, which is composed of the features of the current state and personalized preferences. By linking this reward function to the value function, we can decouple personalized preferences from the dynamics of the MDP. Consequently, we only need to learn the generic features under the current policy, and by merely altering the personalized preferences, we can achieve personalized alignment. Finally, we introduce guided decoding algorithm, which aligns with personalized preferences by utilizing the value function for weighting during the inference phase.


\begin{definition}
\label{personalized reward function}
A \textbf{personalized reward function} R can be represented by:
\begin{equation}
\label{personalized reward function}
    R(p, \bs, \ba) = \bw_p^{\top}\phi(\bs,\ba),
\end{equation}
where $\phi(\bs,\ba) \in \mathbb{R}^d$ are features of current state and action $(\bs,\ba)$ and $\bw_p \in \mathbb{R}^d$ are weights derived from personalized preference 
$p$. 
\end{definition}
Intuitively, $\phi(\bs,\ba)$ can be understood as the salient features (e.g., expert, informative) of the current state, and the vector $\bw_p$ models personalized preferences $p$ as the degree of desirability for each feature. 
\(\bw_p\) is independent of \((\bs,\ba)\). Consequently, when the user's personalized preferences change, only \(\bw_p\) is altered, which in turn modifies the reward function \(R(p, \bs, \ba)\).
% In this manner, \(\bw_p\) is independent of \((\bs,\ba)\), thereby allowing it to be decoupled from the MDP dynamics. When the user's personalized preferences change, only \(\bw_p\) are altered, which in turn modifies the \(R(p, \bs, \ba)\).
% Consequently, the goal of personalized alignment can be defined as obtaining the policy that maximizes the personalized reward for each \(p\).
% To address the resource-intensive nature of existing policy optimization methods, we consider a value-iteration alternative~\citep{watkins1992q} to derive the optimal policy.
We consider derive the value function~\citep{watkins1992q} of personalized reward function, as inspired by that the optimal policy $\pi^*$ obtained by Equation~\ref{eq:multi_step_RL} can be formulated as~\cite{ziebart2010modeling, rafailov2024r}:
\begin{equation}
\label{eq:optimal policy}
    \pi^*(\ba_t|\bs_t, p) = e^{(Q^*(p, \bs_t,\ba_t)-V^*(p, \bs_t))/\beta},
\end{equation}
where $Q$, the action-value function (i.e., Q function) based on the token-level reward $R^{\pi}(p, \bs, \ba)$, models the total future reward from $(\bs, \ba)$ under policy $\pi$. $V$ is the corresponding state-value function at current state that $V^{\pi}(p, \bs_t) = \beta \log \left( \int_{\mathcal{A}} e^{Q^{\pi}(p, \bs_t, \ba_t)/\beta} \, d\ba \right)$. Q function can be expressed as:
\begin{align}
    Q^{\pi}(p, \bs_t, \ba_t) &= \mathbb{E} [\sum_{i=t}^{T} R(p, \bs_i,\ba_i)| \ba_i \sim \pi (\cdot|\bs_i)], \label{eq:Q_function}
\end{align}
where $\mathbb{E}$ is the expectation is over the randomness due to the sampling from the base language model $\pi$. $Q^*$ denotes the Q funtion under optimal policy $\pi^{*}$.
Substitute Eq.~\ref{personalized reward function} into Eq.~\ref{eq:Q_function}, we can express $Q$ function as:
\begin{align}
\label{personalized Q}
    Q^{\pi}(p, \bs_t, \ba_t) &= \bw_p^{\top} \mathbb{E} [\sum_{i=t}^{T} \phi(\bs_i,\ba_i)| \ba_i \sim \pi (\cdot|\bs_i)] = \bw_p^{\top} \psi^{\pi}(\bs_t, \ba_t).
\end{align}

To obtain the $Q^*$ function, we begin by rewrite Eq.~\ref{eq:optimal policy} as in \citet{rafailov2024direct}:
\begin{equation}
\label{rewriteR}
\sum_{t=1}^T R (p, \bs_t, \ba_t) = \sum_{t=1}^T \beta \text{log}\frac{{\pi}_{\theta}(\ba_t|\bs_t, p)}{{\pi}_{\text{ref}}(\ba_t|\bs_t, p)} + V^*(\bs_0).\\
\end{equation}
Denote $\text{log}\hat{\pi}(\ba|\bs)$ as the features of $(\bs,\ba)$, that satisfies $\text{log}{\pi}(\ba|\bs, p) = \bw_p^{\top}\text{log}\hat{\pi}(\ba|\bs)$. Substitute this relationship and Eq.~\ref{rewriteR} into Eq.~\ref{eq:reward modeling}, we can derive the loss function for personalized reward modeling:
\begin{equation}
\label{finalloss}
\mathcal{L}_{\text{PRM}}(\pi_{\theta}, D) = -\mathbb{E}_{(\bx, \by_w, \by_l) \sim D} \left[ \log \sigma \left( \bw_p^{\top} (\sum_{t=1}^{T}\beta\log\frac{\hat{\pi}_{\theta}(\ba^w_t|\bs^w_t)}{\hat{\pi}_{\text{ref}}(\ba^w_t|\bs^w_t)} -\sum_{t=1}^{T}\beta\log\frac{\hat{\pi}_{\theta}(\ba^l_t|\bs^l_t)}{\hat{\pi}_{\text{ref}}(\ba^l_t|\bs^l_t)}) \right) \right].
\end{equation}
Inspired by \citet{rafailov2024direct}, we can derive implicit Q function $Q^{*}(p, \bs_t, \ba_t)$ with token-level reward $\bw_p^{\top}\beta \text{log}(\hat{\pi}^{*}_{\theta}(\ba_i | \bs_i)- \hat{\pi}_{\text{ref}}(\ba_i | \bs_i)$:
\begin{equation}
\label{Qfunction}
Q^{*}(p, \bs_t, \ba_t) =  \bw_p^{\top}\psi^{*}(\bs_t, \ba_t) = \bw_p^{\top} \beta \sum_{i=1}^{t} \log \frac{\hat{\pi}^{*}_{\theta}(\ba_i | \bs_i)}{\hat{\pi}_{\text{ref}}(\ba_i | \bs_i)}+V^{*}(p, \bs_1). \\
\end{equation}

Then, we formulate personalized alignment as decoding-time $Q^*$ guided search according to Eq.~\ref{eq:optimal policy}.

\begin{definition}
\textbf{Personalized alignment at decoding-time (\model)}: The optimal policy $\pi_{\model}^*$ of personalized alignment can be defined as selecting the action for the base model $\pi_{LM}$ that maximizes the advantage function $Q^{*}(p,\bs_t,\ba)-V^{*}(p,\bs_t)$ towards certain personalized preference $p$ at each step:
\begin{align}
\label{modelfuntion}
    \pi_{\model}^*(\ba | \bs_t, p) & \propto \pi_{LM}(\ba | \bs_t) e^{\beta(Q^{*}(p,\bs_t,\ba)-V^{*}(p,\bs_t))}.
\end{align}
\end{definition}

The detailed derivations are provided in the appendix~\ref{sec:Optimal Q function}. Note that different from RLHF framework that directly models the language model as policy, our PAD policy $\pi_{\model}$ is different from the base language model $\pi_{LM}$, as well as the personalized reward model $\pi_{\theta}$.

\begin{figure}[t]
	\centering
	\includegraphics[width=1.\linewidth]{fig/Personalized_Decoding_Pipeline2.pdf}
	\caption{An illustration of the inference phase for personalized alignment at decoding-time (PAD). The corresponding description can be found in Sec.~\ref{sec:Practical Implementations}.}
    \label{fig:pipeline}
\end{figure}


\subsection{Generalized personalized alignment}

In this section, we discuss the ability of~\model~to transfer to unseen personalized preferences. Suppose now that we have computed optimal value function for n personalized preferences \(\bw_1, \bw_2, \ldots, \bw_n \in \bw^\phi\), denoted as \(\{Q^{*}_{1}, Q^{*}_{2}, \ldots, Q^{*}_{n}\}\).
Now, if the reward changes to $R(p_{n+1},\bs,\ba) = \bw_{n+1}^\top \phi(\bs,\ba) $, as long as we have $\bw_{n+1}$ we can compute the new value function of $\pi_i^*$ by simply making $Q_{n+1}^{*}(\bs,\ba) = \bw_{n+1}^\top \psi^{*}(\bs,\ba) $. Once the functions $Q_{n+1}^{*}$ have been computed, we can we can apply generalized policy improvement~\citep{bellman1966dynamic, barreto2017successor} to estimate its performance on $\bw_{n+1}$.


\textbf{Theorem 1.} Let $\bw_i \in \mathcal{W}^\phi$ and let $Q_i^{*}$ be the action-value function of an optimal policy of $\bw_i$. 
for all $\bs \in \mathcal{S}$, $\ba \in \mathcal{A}$, and $j \in \{ 1, 2, \dots, n \}$, let $\pi(\bs) \in \arg\max_a \max_i Q_i^{*}(\bs, \ba)$. Finally, let $\phi_{\max} = \max_{\bs,\ba} \| \phi(\bs,\ba) \|$, where $\| \cdot \|$ is the norm induced by the inner product adopted. Then,
\begin{equation}
    Q_{n+1}^{\pi^*}(p_{n+1}, \bs, \ba) - Q_{n+1}^{\pi}(p, \bs, \ba) \leq |H| \left( \phi_{\max} \min_j \| \mathbf{w}_{p_{n+1}} - \mathbf{w}_{p_j} \|\right).
\end{equation}
This term is a multiple of the distance between \(\bw_i\) and the closest \(\bw_j\) for which we have already computed a policy. The formula formalizes the intuition that if the agent has previously solved a similar task, it should perform well on task \(\bw_i\). The proofs of Theorem 1 are in the Appendix~\ref{sec:Generalized personalized alignment}.




\subsection{Practical Implementations}
\label{sec:Practical Implementations}

In this section, we introduce the practical implementation of Personalized Alignment at Decoding-time (PAD), which includes the optimization of the personalized reward model and the inference-time guided decoding.


\paragraph{Optimization}
As previously mentioned, we can decouple personalized preferences from the MDP process during the personalized alignment procedure.
Thus, we consider utilizing an LLM-based model as a personalized reward model (PRM) $\pi_\theta$ to independently predict the features $\phi(\bs,\ba)$ and preferences $\bw_p$. For simplicity, we employ a single backbone to predict the embeddings for both $\phi(\bs,\ba)$ and $p$ and then utilize an additional value head to predict $\bw_p$. The optimization occurs in two stages with Equation~\ref{finalloss}. In the first stage, we fix $\bw_p$ as a unit vector and optimize the backbone to learn general features. In the second stage, we freeze the backbone and only optimize the value head for $\bw_p$ to learn different user preferences. The optimized PRM is denoted as $\pi^{*}_\theta$.



\paragraph{Guided Decoding}
The inference phase of PAD is shown in Figure~\ref{fig:pipeline}. Given the personalized preference $p$ and the previous context $s = (x, y_{<t})$ at step $t$, we first calculate the predicted probability distribution of the base model $\pi_{LM}(\ba | \bs_t)$ for the next token $\ba$. Then we calculate the reward from PRM by $R(p,\bs_t,\ba) = \bw_p^{\top}\phi(\bs_t,\ba) = \bw_p^{\top}  \log \hat{\pi}^{*}_{\theta}(\ba | \bs_t)-{\hat{\pi}_{\text{ref}}(\ba_t | \bs_t)}$ for the token.
Finally, $\ba_t$ can be selected from their weighted sum:
\begin{align}
\label{eq:Guided Decoding}
\pi^*_{\text{\model}}(\ba_t | \bs_t, p) := \arg\max_{\ba} \mathbb{E}_{\ba \sim \pi_{LM}(\cdot | \bs_t)} \text{exp}\left[  \beta \bw_p^{\top}  \log \frac{\hat{\pi}^{*}_{\theta}(\ba | \bs_t)}{\hat{\pi}_{\text{ref}}(\ba | \bs_t)}  + \pi_{LM}(\ba | \bs_t)\right].
\end{align}
Eq.~\ref{eq:Guided Decoding} is equivalent to Eq.~\ref{modelfuntion}, with proofs in the appendix~\ref{sec:Optimal Q function}. Note that $\beta$ in Eq.~\ref{eq:Guided Decoding} is also treated as a weight hyperparameter for simplicity, which slightly differs from its previous definition.


==> tex/4_exp.tex <==


\section{Experiment}
\subsection{Experiment Setup}
\subsubsection{\model~Setup}
During the development of our personalized reward model, we utilized datasets from multiple sources including Ultrafeedback~\citep{cui2023ultrafeedback}, HelpSteer2~\citep{wang2024helpsteer2}, Rewards-in-Context~\citep{yang2024rewards}, and SafeRLHF~\citep{dai2023safe}.  
To simulate personalized preferences, synthetic user prompts are prepended to instructions, following \citet{jang2023personalized}.
We employ the Llama-3-8B model~\citep{llama3modelcard} as our backbone, and append a linear layer directly following the embeddings, featuring an output dimension of 4096. Comprehensive details on the datasets, the pre-processing process and the implementations are documented in Appendix~\ref{sec: PAD Details}.
During the decoding phase, we utilize greedy decoding with top-$k$ candidates. We restrict the maximum lengths of the initial prompt and subsequent generations to 2,048 and 128 tokens, respectively. The hyperparameters $k=10$, are optimized to maximize the average reward performance observed in our validation datasets. An exhaustive analysis of the decoding strategies and hyperparameter settings is provided in Section~\ref{sec:Decoding Strategy}.
\subsubsection{Evaluation Setup}

\paragraph{Datasets and base models.} We utilize two evaluation datasets. The P-Soups~\citep{jang2023personalized} evaluation dataset has been filtered and modified based on the Koala evaluation by \citet{jang2023personalized}. The HelpSteer2~\citep{wang2024helpsteer2} (validation split) dataset is a multi-aspect alignment dataset comprising 1,000 prompts. In our evaluation setup, we initially focus on alignment the three pre-defined dimensions: `harmless', `helpful', and `humor', following previous works~\citep{yang2024rewards, yang_metaaligner_2024, shi2024decoding}. Additionally, to assess the scalability of the Personalized Alignment Dataset (\model), we simulate users each having unique personalized preferences drawn from several preference dimensions, collectively forming 12 preference combinations.
For personalized alignment, we primarily utilize
\revise{Llama-3-8B-SFT}~\citep{llama3modelcard, meng2024simposimplepreferenceoptimization} as the base language model. Additional experiments are conducted on Gemma~\citep{gemma_2024}, Mistral-7B-SFT~\citep{jiang2023mistral7b,tunstall2023zephyrdirectdistillationlm}, and Llama-2~\citep{touvron2023llama2openfoundation} to test scalability.
\paragraph{Evaluation metrics.}
For the evaluation of `harmless', `helpful', and `humor' dimensions, we integrate three open-source reward models available on Huggingface, as delineated by \citet{yang2024rewards, yang_metaaligner_2024}. Additionally, we employ the ArmoRM \citep{wang2024interpretable}, a multi-dimension reward model known for its state-of-the-art performance on the Reward-Bench benchmark \citep{RewardBench}. For these reward models, we report their scores assessing LLM responses from various perspectives.
Furthermore, our evaluation leverages GPT-4, a widely recognized tool in previous studies \citep{khanov2024args, yang_metaaligner_2024}, to conduct the judgments towards certain personalized preference and report the win rate. Comprehensive details on the evaluation metrics, reward models and GPT-4 judgments are provided in Appendix \ref{app:Evaluation Details}.

\paragraph{Baselines.}
We compare~\model~with 9 personalized alignment or multi-objective alignment methods as delineated in Table~\ref{tab:method_comparison}. MORLHF~\citep{li2020deep} optimizes for the weighted multi-objective reward function using PPO. MODPO~\citep{zhou2023beyond} integrates language modeling with reward modeling, training models to combine all objectives with specific weights. Personalized soups~\citep{jang2023personalized} first optimizes multiple policy models and then merges the parameters of the policy models according to preference. Rewarded soup~\citep{rame2024rewarded} first trains multiple  specializing networks independently, and then interpolates their weights linearly. Rewards-in-Context (RiC)~\citep{yang2024rewards} conditions foundation model responses on multiple rewards in its prompt and uses supervised fine-tuning for alignment. MetaAligner~\citep{yang_metaaligner_2024} and \revise{Aligner}~\citep{ji2024aligner} train an additional model to perform conditional weak-to-strong correction. Preference prompting~\citep{jang2023personalized} simply prompts for preferences without any additional training. MOD~\citep{shi2024decoding} first trains multiple specializing networks and performs linear combination of their predictions. \revise{Steering~\citep{konen2024style} adjusts the output of LLMs by adding style vectors
 to the activations of hidden layers.} 
Args~\citep{khanov2024args} is a reward-guided decoding-time alignment framework. 
%As Args is originally designed for general preference, we use ArmoRM~\citep{wang2024interpretable} to provide rewards.

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{fig/soup.pdf}
        \caption{Alignment results on P-Soups dataset.}
        \label{fig:sub1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{fig/steer.pdf}
        \caption{Alignment results on HelpSteer2 dataset.}
        \label{fig:sub2}
    \end{subfigure}
    \caption{Alignment results for pre-defined preferences related to harmless, helpful, and humor.}
    \label{fig:Alignment on predefined}
\end{figure}

\subsection{Main Results}
\label{sec: main results}

\paragraph{Alignment on Pre-defined Preferences}
We initiate our evaluation by focusing on three pre-defined dimensions seen in the training phase: `harmless', `helpful', and `humor'. As depicted in Figure~\ref{fig:Alignment on predefined}, each point represents the average rewards corresponding to specific user preferences, encompassing either single or dual dimensions, evaluated across two distinct datasets. We dynamically adjust the weights of these dimensions for the baseline models. The results demonstrate that PAD can effectively align with various preferences, outperforming the baselines in terms of achieving a superior frontier. 
Subsequently, we compare the performance of PAD with baseline methods in aligning to the three dimensions simultaneously. For baselines, we set uniform preference weights for three dimensions. The performance of PAD across two datasets is presented in Table~\ref{tab:methods_evaluation}. 
The findings reveal that PAD has achieved substantial improvements for all three objectives. Within the P-Soups dataset, PAD achieves an average win rate of 84\%, elevating the average score of the reward model from 0.32 to 1.06. Across all eight rewards or win rates, PAD surpasses all baselines in six metrics. On the HelpSteer2 evaluation dataset, PAD achieves the best in seven out of eight metrics and significantly enhances overall personalized preference alignment performance. These results demonstrate the superiority of PAD in personalized alignment.

\input{tab/method_evaluation}



% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.8\linewidth]{fig/radar.pdf}
% 	\caption{Alignment results on two datasets with normalized harmless, helpful, and humor rewards. \wchai{too ugly :((( }}
%  \label{fig:Alignment on predefined}
% \end{figure}

\begin{figure}[t]
	\centering  %图片全局居中
	\includegraphics[width=1.0\linewidth]{fig/customized_preference2.pdf}
	\caption{Alignment on Customized Preferences. Abbreviations include "Exp" for Expert, "Inf" for Informative, "Cre" for Creative, "Pre" for Preliminary, "Con" for Concise, and "Fac" for Factual.}
    \label{fig:customized}
\end{figure}

\paragraph{Alignment on Customized Preferences}
In previous experiments, we were limited to aligning with pre-defined preferences. As previously noted, most existing methods focus on aligning with preferences or dimensions defined during the training phase. However, in real-world personalization scenarios, there still exist diverse unseen personalized preferences, which current methods struggle to address. Considering this aspect, we evaluate the ability of alignment on customized preferences in this part. 
We additionally define three dimensions `expert', `informative', and `creative' that were unseen during the training phase, which result in 8 personalized preferences. We compare the alignment performance of PAD with preference prompting and MetaAligner on the P-soups dataset. The GPT-4 judgment results between the generations of different methods and Llama-3-Base are provided in Figure~\ref{fig:customized}. As can be seen, PAD consistently improves win rate across all eight types of personalized preferences, outperforming both baselines. This confirms the superiority of PAD in generalizing to unseen personalized preferences.

\subsection{Decoding Strategy}
\label{sec:Decoding Strategy}

\paragraph{Sensitivity Analysis on Decoding Hyperparameters}
In our initial analysis, we investigate the impact of adjusting the hyperparameters $\beta$ and $k$ on the performance of reward models within the P-Soups dataset. Additionally, we incorporate a diversity score as a metric. A higher diversity score indicates an enhanced capability to generate texts with a broader variety of vocabulary, as detailed in Appendix~\ref{app:Evaluation Details}.
The results are illustrated in Figure~\ref{fig:Sensitivity analysis on beta}. It is evident that increasing the weighting parameter $\beta$ leads to a rise in reward scores. However, beyond a certain threshold, the scores for helpfulness and harmlessness begin to diminish, suggesting that excessively elevated $\beta$ values might lead the generation process to deviate substantially from the base model's core knowledge, thereby compromising its intrinsic qualities. Concurrently, as $\beta$ increases, there is a slight increase in diversity, indicating that higher $\beta$ values encourage the generation of a more varied vocabulary. Regarding the number of candidates $k$, the performance depicted in Figure~\ref{fig:Sensitivity analysis on k} suggests that a larger number of candidates may slightly encourage the generation of more diverse responses. However, it has minimal impact on producing more personalized-aligned responses.

% This analysis underscores the nuanced interplay between hyperparameter settings and model performance in terms of both generating diverse content and aligning with specific user preferences.

\begin{wrapfigure}{r}{0.5\textwidth}
	\centering
    \vspace{-24pt}
	\includegraphics[width=1\linewidth]{fig/Strategy.pdf}
	\caption{Comparison of various decoding strategies that can be integrated with our PAD.}
    \vspace{-6pt}
    \label{fig:decoding strategies}
\end{wrapfigure}
\paragraph{Effect of Decoding strategies.}

We compare the performance with three decoding strategies, which can be integrated with our PAD. (1) Greedy: select the token with maximum score. (2) Stochastic: sample a token from the probability distribution of the top-k candidate. (3) Best-of-k: generate k responses from the base model and select the one with maximum score. The temperature parameter is set to be 0.7 for stochastic and best-of-k and k is set to 10 for all strategies. Additionally, we compared the performance with (4) Base: greedy generation using only the base model as a reference.
The average scores and standard deviations for the reward model and diversity across three runs, are illustrated in Figure~\ref{fig:decoding strategies}. For clarity in visualization, humor scores below zero have been clipped. It is evident that all three decoding strategies enhance alignment. In some dimensions, stochastic and best-of-k strategies achieve better alignment than greedy, demonstrating the effectiveness of exploration. However, their performance variance is high, indicating some instability. Regarding diversity, all strategies show marginal improvements. 

\paragraph{\revise{Computational Cost for PAD}}
\revise{
Building on the previous section, we evaluate the computational costs of decoding-time alignment, with results detailed in Table~\ref{tab:decoding strategies}, which is measured on a single NVIDIA H100 GPU. The time costs for training-based models closely align with those of the `Base' configuration. Our results reveal that generation time of PAD increases by 2-3 times compared with conventional greedy decoding. Additionally, we have quantified the memory overhead of PAD. Decoding with PAD requires an additional 17,095 MB.
Despite this increase in processing time and memory, there is a notable enhancement in performance across all dimensions (e.g., 26\% increase as for `helpful'), indicating a reasonable tradeoff between alignment performance and inference speed.}


\begin{figure}[t]
    \centering
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[height=4cm]{fig/beta.pdf}
        \caption{Sensitivity analysis on $\beta$.}
        \label{fig:Sensitivity analysis on beta}
    \end{minipage}\hfill
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[height=4cm]{fig/k.pdf}
        \caption{Sensitivity analysis on $k$.}
        \label{fig:Sensitivity analysis on k}
    \end{minipage}
\end{figure}

% \begin{table}[t]
% \centering
% \caption{Scalability on different base models.}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Base Model} & \textbf{Helpful} & \textbf{Harmless} & \textbf{Humor} \\
% \midrule
% Gemma-2b-it   & 0.9833 & 0.6782 & -0.097  \\
% $+$\model        & 1.3693 & 0.9347 & -0.5325 \\
% Mistral-7B-SFT  & 1.5887 & 0.7777 & -0.9582 \\
% $+$\model        & 1.6747 & 0.9589 & 0.9351  \\
% llama-2-7b-chat & 0.6326 & 0.9509 & 1.3861  \\
% $+$\model        & 0.861  & 1.1368 & 1.0875  \\
% \bottomrule
% \end{tabular}
% \label{tab:model_metrics}
% \end{table}

\begin{table*}[t]
\caption{Analysis of PAD scalability across various base models.}
\centering
  \resizebox{0.98\textwidth}{!}{
  \begin{tabular}{l|c|ccc|ccc|cc|cc}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{w}&\multicolumn{3}{c}{Helpful} & \multicolumn{3}{|c}{Harmless} & \multicolumn{2}{|c}{Humor} & \multicolumn{2}{|c}{Overall} \\
    \cmidrule(r){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
            & & Armo & RM &GPT-4  & Armo & RM &GPT-4  & RM &GPT-4  & RM & GPT-4 \\
    \hline
Gemma-2b-it     & -   & 0.98 & 0.47 & -     & 0.68 & 0.96 & -     & -0.10         & -     & 0.44 & -     \\
w/ \model           & 0.8 & \textbf{1.37} & \textbf{0.50} & 64\%  & \textbf{0.93} & \textbf{0.99} & 100\% & \textbf{0.53}          & 72\%  & \textbf{0.67} & 79\%  \\
Mistral-7b-SFT  & -   & 1.59 & 0.58 & -     & 0.78 & 0.97 & -     & -0.95         & -     & 0.20 & -     \\
w/ \model            & 0.2 & \textbf{1.67} & \textbf{0.60} & 54\%  & \textbf{0.96} & \textbf{1.00} & 92\%  & \textbf{0.93} & 78\%  & \textbf{0.84} & 75\%  \\
Llama-2-7b-chat & -   & 0.63 & 0.47 & -     & 0.95 & 0.91 & -     & \textbf{1.38}          & -     & \textbf{0.92} & -     \\
w/ \model            & 0.2 & \textbf{0.86} & \textbf{0.48} & 82\%  & \textbf{1.14} & \textbf{0.93} & 100\% & 1.08          & 56\%  & 0.83 & 79\%  \\
Llama-3-8b-it   & -   & 1.06 & 0.65 & -     & 0.75 & \textbf{0.99} & -     & 1.59          & -     & 1.08 & -     \\
w/ \model            & 1.0 & \textbf{1.38} & \textbf{0.68} & 82\%  & \textbf{1.02} & \textbf{0.99} & 96\%  & \textbf{1.97}          & 76\%  & \textbf{1.21} & 85\% 
 \\\bottomrule
  \end{tabular}}
  \label{tab:different base models}
\end{table*}


\subsection{Model-agnostic Analysis}
\revise{In this section, we explore the scalability of PAD to a broader range of base models. We employ the same personalized reward model, which does not require retraining for different base models.}
% We further apply PAD to a broader range of base models to verify its scalability and model-agnostic properties across different base models. 
As illustrated in Table~\ref{tab:different base models}, PAD significantly enhances the personalized alignment performance of models across a diverse spectrum of models, demonstrating its model-agnostic nature. In comparison with other methods that require retraining of the policy model (i.e., the language model), our approach requires only the training of a reward model to achieve model-agnostic personalized alignment. This highlights the superiority of our PAD.

% Additionally, we report the $\beta$ values across different base models when achieving optimal alignment. Compared to Llama-3, the $\beta$ values for other models are considerably lower, and the performance improvements are not as pronounced. \revise{This may be attributed to variations in the vocabulary and MDP dynamics between the base model and the reward model, leading to imprecise estimates of personalized rewards.}

